Transformer Quality in Linear Time

We revisit the design choices in Transformers, and propose methods to address their weaknesses in handling long sequences. First, we propose a simple layer named gated attention unit, which allows the use of a weaker single-head attention with minimal quality loss. We then propose a linear approximation method complementary to this new layer, which is accelerator-friendly and highly competitive in quality. The resulting model, named FLASH, matches the perplexity of improved Transformers over both short (512) and long (8K) context lengths, achieving training speedups of up to 4.9$\times$ on Wiki-40B and 12.1$\times$ on PG-19 for auto-regressive language modeling, and 4.8$\times$ on C4 for masked language modeling.

==> Transformer Quality in Linear time/lm_wiki_fig.tex <==
\begin{figure*}[ht]
\centering     %
\vspace{-0.5cm}
\resizebox{1.0\textwidth}{!}{
\subfigure
{
    \label{fig:lm_legend}
    \includegraphics[ width=0.35\textwidth]{figures/legend.pdf}
}
}
\vspace{-0.8cm}
\\
\setcounter{subfigure}{0}
\resizebox{\textwidth}{!}{
\subfigure[Per-step training latency]
{
    \label{fig:lm_wiki_lat}
    \includegraphics[width=0.32\textwidth]{figures/lm_wiki_lat.pdf}
}%
\subfigure[Context length = 512]
{
    \label{fig:lm_wiki_s512}
    \includegraphics[width=0.33\textwidth]{figures/lm_wiki_s512.pdf}
}%
\subfigure[Context length = 1024]
{
    \label{fig:lm_wiki_s1024}
    \includegraphics[ width=0.33\textwidth]{figures/lm_wiki_s1024.pdf}
}
}
\\
\resizebox{\textwidth}{!}{
\subfigure[Context length = 2048]
{
    \label{fig:lm_wiki_s2048}
    \includegraphics[width=0.33\textwidth]{figures/lm_wiki_s2048.pdf}
}%
\subfigure[Context length = 4096]
{
    \label{fig:lm_wiki_s4096}
    \includegraphics[width=0.33\textwidth]{figures/lm_wiki_s4096.pdf}
}%
\subfigure[Context length = 8192]
{
    \label{fig:lm_wiki_s8192}
    \includegraphics[ width=0.33\textwidth]{figures/lm_wiki_s8192.pdf}
}
}
\caption{Auto-regressive language modeling validation-set results on the Wiki-40B dataset --- \small{All models are sized around 110M (i.e., BERT-Base scale) and trained for 125K steps with 2$^{18}$ tokens per batch. The quality is measured in negative log perplexity.}}
\label{fig:lm}
\end{figure*}

==> Transformer Quality in Linear time/mlm_c4_fig.tex <==
\begin{figure*}[!ht]
\centering     %
\vspace{-0.5cm}
\resizebox{1.0\textwidth}{!}{
\subfigure
{
    \label{fig:mlm_legend}
    \includegraphics[ width=0.35\textwidth]{figures/legend.pdf}
}
}
\vspace{-0.8cm}
\\
\setcounter{subfigure}{0}
\resizebox{\textwidth}{!}{
\subfigure[Per-step training latency]
{
    \label{fig:mlm_c4_lat}
    \includegraphics[height=4 cm, width=0.31\textwidth]{figures/mlm_c4_lat.pdf}
}%
\subfigure[Context length = 512]
{
    \label{fig:mlm_c4_s512}
    \includegraphics[height=4.22 cm, width=0.33\textwidth]{figures/mlm_c4_s512.pdf}
}%
\subfigure[Context length = 1024]
{
    \label{fig:mlm_c4_s1024}
    \includegraphics[height=4.22 cm, width=0.33\textwidth]{figures/mlm_c4_s1024.pdf}
}
}
\\
\resizebox{\textwidth}{!}{
\subfigure[Context length = 2048]
{
    \label{fig:mlm_c4_s2048}
    \includegraphics[height=4.22 cm, width=0.33\textwidth]{figures/mlm_c4_s2048.pdf}
}%
\subfigure[Context length = 4096]
{
    \label{fig:mlm_c4_s4096}
    \includegraphics[height=4.22 cm, width=0.33\textwidth]{figures/mlm_c4_s4096.pdf}
}%
\subfigure[Context length = 8192]
{
    \label{fig:mlm_c4_s8192}
    \includegraphics[height=4.22 cm, width=0.33\textwidth]{figures/mlm_c4_s8192.pdf}
}
}
\caption{Masked language modeling validation-set results on the C4 dataset --- \small{All models are comparable in size at around 110M (i.e., BERT-Base scale) and trained for 125K steps with 2$^{18}$ tokens per batch. The quality is measured in negative log perplexity.}}
\label{fig:mlm}
\end{figure*}
